Bodyseismography (BSG): Theoretical Foundation and Numerical Modeling

Bodyseismography (BSG) records cardiovascular vibrations transmitted through the body and a supporting bed, enabling contactless assessment of cardiac mechanics. Relating these vibrations to hemodynamic features requires separating cardiac excitation from the effects of body and bed transmission. We develop a source-transmission-measurement framework that couples myocardial contraction and vascular recoil to directional BSG observations. The theory connects stroke volume, cardiac output, and blood pressure to observation and target Jacobians, establishes a local first-order target-observability criterion, and characterizes how additional sensing axes reduce ambiguities under specified source and transmission uncertainties. Numerical modeling combines four-chamber cardiac mechanics, cardiac-to-body excitation, and calibrated body-bed operators. Across 27 participants, a multilayer finite-element model with calibrated frequency correction achieves median Pearson correlation coefficients of 0.865 for the vertical channel and 0.682 for the planar-sum channel in matched-window waveform reconstruction. Controlled stroke-volume perturbations show that transmission reshapes feature sensitivity, including a reversal of the vertical feature association in 8 of 27 participant-specific transfer models. These analytical and numerical studies explain how cardiovascular sources and mechanical propagation jointly shape triaxial BSG and provide a physical basis for relating directional vibration features to hemodynamic changes.

==> figures/signals/scg_valve_cycle.tex <==
%
%
\begingroup
\newcommand{\SCGheart}[3]{%
\begin{tikzpicture}[x=0.64cm,y=0.64cm,line cap=round,line join=round]
\path[use as bounding box] (-0.95,-0.10) rectangle (0.90,2.45);
%
\path[draw=black!75,fill=red!18,line width=0.65pt]
 (-0.43,1.36) .. controls (-0.87,0.97) and (-0.42,0.21) .. (0.05,0.02)
 .. controls (0.36,0.15) and (0.64,0.91) .. (0.45,1.38)
 .. controls (0.24,1.56) and (-0.17,1.54) .. cycle;
\path[fill=white,draw=black!55,line width=0.4pt]
 (-0.30,1.25) .. controls (-0.57,0.91) and (-0.24,0.36) .. (0.06,0.18)
 .. controls (0.24,0.38) and (0.46,0.98) .. (0.31,1.27) -- cycle;
\path[draw=black!70,fill=red!8,line width=0.6pt]
 (-0.30,1.28) -- (-0.30,1.48)
 .. controls (-0.69,1.58) and (-0.62,2.03) .. (-0.10,2.06)
 .. controls (0.30,2.05) and (0.30,1.62) .. (0.09,1.49) -- (0.09,1.28);
\path[draw=black!70,fill=red!8,line width=0.6pt]
 (0.22,1.23) -- (0.22,2.22) -- (0.52,2.22) -- (0.52,1.23);
%
\ifnum#1=1
 \draw[navy,line width=1pt] (-0.30,1.38)--(-0.25,1.10) (0.09,1.38)--(0.03,1.10);
 \draw[-{Stealth[length=2.3pt]},red!65!black,line width=0.8pt] (-0.10,1.72)--(-0.10,0.80);
\else
 \draw[navy,line width=1pt] (-0.30,1.38)--(-0.105,1.26)--(0.09,1.38);
\fi
%
\ifnum#2=1
 \draw[navy,line width=1pt] (0.22,1.63)--(0.25,1.84) (0.52,1.63)--(0.49,1.84);
 \draw[-{Stealth[length=2.3pt]},red!65!black,line width=0.8pt] (0.37,1.15)--(0.37,2.30);
\else
 \draw[navy,line width=1pt] (0.22,1.63)--(0.37,1.51)--(0.52,1.63);
\fi
%
\foreach \sx/\sy/\ex/\ey in {
 -0.52/1.03/-0.30/0.99,
 -0.36/0.57/-0.18/0.67,
  0.49/1.02/0.28/0.99,
  0.32/0.57/0.16/0.67,
 -0.11/0.26/-0.035/0.43,
  0.145/0.26/0.105/0.44}{
 \ifnum#3=1
  \draw[-{Stealth[length=1.8pt,width=1.7pt]},black,line width=0.65pt]
    (\sx,\sy)--(\ex,\ey);
 \else
  \draw[-{Stealth[length=1.8pt,width=1.7pt]},black,line width=0.65pt]
    (\ex,\ey)--(\sx,\sy);
 \fi
}
\end{tikzpicture}}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}cccc@{}}
\SCGheart{0}{0}{1}&\SCGheart{0}{1}{1}&\SCGheart{0}{0}{0}&\SCGheart{1}{0}{0}\\[-2pt]
\makebox[0.238\linewidth]{\scriptsize\textbf{MC}}&
\makebox[0.238\linewidth]{\scriptsize\textbf{AO}}&
\makebox[0.238\linewidth]{\scriptsize\textbf{AC}}&
\makebox[0.238\linewidth]{\scriptsize\textbf{MO}}
\end{tabular}\par
\endgroup


==> figures/signals/scg_waveform_coordinates.tex <==
\draw[black,line width=0.65pt,line cap=round,line join=round] plot coordinates {
(-248.63782,0.57208)
(-247.95673,0.57208)
(-247.27564,0.57208)
(-246.59455,0.57208)
(-245.91346,0.57208)
(-245.23237,0.57208)
(-244.55128,0.57208)
(-243.87019,0.57208)
(-243.18910,0.57208)
(-242.50801,0.57208)
(-241.82692,0.57208)
(-241.14583,0.57208)
(-240.46474,0.57208)
(-239.78365,0.45767)
(-239.10256,0.45767)
(-238.42147,0.45767)
(-237.74038,0.45767)
(-237.05929,0.45767)
(-236.37821,0.45767)
(-235.69712,0.45767)
(-235.01603,0.45767)
(-234.33494,0.45767)
(-233.65385,0.34325)
(-232.97276,0.34325)
(-232.29167,0.34325)
(-231.61058,0.34325)
(-230.92949,0.34325)
(-230.24840,0.34325)
(-229.56731,0.34325)
(-228.88622,0.34325)
(-228.20513,0.34325)
(-227.52404,0.34325)
(-226.84295,0.34325)
(-226.16186,0.34325)
(-225.48077,0.34325)
(-224.79968,0.34325)
(-224.11859,0.34325)
(-223.43750,0.34325)
(-222.75641,0.34325)
(-222.07532,0.34325)
(-221.39423,0.34325)
(-220.71314,0.22883)
(-220.03205,0.34325)
(-219.35096,0.34325)
(-218.66987,0.34325)
(-217.98878,0.34325)
(-217.30769,0.34325)
(-216.62660,0.34325)
(-215.94551,0.34325)
(-215.26442,0.34325)
(-214.58333,0.34325)
(-213.90224,0.34325)
(-213.22115,0.34325)
(-212.54006,0.34325)
(-211.85897,0.34325)
(-211.17788,0.34325)
(-210.49679,0.34325)
(-209.81571,0.34325)
(-209.13462,0.34325)
(-208.45353,0.34325)
(-207.77244,0.34325)
(-207.09135,0.34325)
(-206.41026,0.34325)
(-205.72917,0.22883)
(-205.04808,0.22883)
(-204.36699,0.22883)
(-203.68590,0.22883)
(-203.00481,0.22883)
(-202.32372,0.22883)
(-201.64263,0.22883)
(-200.96154,0.22883)
(-200.28045,0.22883)
(-199.59936,0.22883)
(-198.91827,0.22883)
(-198.23718,0.22883)
(-197.55609,0.22883)
(-196.87500,0.22883)
(-196.19391,0.22883)
(-195.51282,0.22883)
(-194.83173,0.22883)
(-194.15064,0.22883)
(-193.46955,0.22883)
(-192.78846,0.22883)
(-192.10737,0.22883)
(-191.42628,0.22883)
(-190.74519,0.22883)
(-190.06410,0.22883)
(-189.38301,0.11442)
(-188.70192,0.11442)
(-188.02083,0.11442)
(-187.33974,0.11442)
(-186.65865,0.11442)
(-185.97756,0.11442)
(-185.29647,0.11442)
(-184.61538,0.11442)
(-183.93429,0.11442)
(-183.25321,0.11442)
(-182.57212,0.11442)
(-181.89103,0.11442)
(-181.20994,0.22883)
(-180.52885,0.22883)
(-179.84776,0.22883)
(-179.16667,0.22883)
(-178.48558,0.22883)
(-177.80449,0.22883)
(-177.12340,0.22883)
(-176.44231,0.22883)
(-175.76122,0.22883)
(-175.08013,0.22883)
(-174.39904,0.22883)
(-173.71795,0.22883)
(-173.03686,0.22883)
(-172.35577,0.22883)
(-171.67468,0.22883)
(-170.99359,0.22883)
(-170.31250,0.22883)
(-169.63141,0.22883)
(-168.95032,0.22883)
(-168.26923,0.22883)
(-167.58814,0.22883)
(-166.90705,0.11442)
(-166.22596,0.11442)
(-165.54487,0.11442)
(-164.86378,0.11442)
(-164.18269,0.11442)
(-163.50160,0.11442)
(-162.82051,0.11442)
(-162.13942,0.11442)
(-161.45833,0.11442)
(-160.77724,0.11442)
(-160.09615,0.22883)
(-159.41506,0.22883)
(-158.73397,0.22883)
(-158.05288,0.22883)
(-157.37179,0.22883)
(-156.69071,0.22883)
(-156.00962,0.22883)
(-155.32853,0.22883)
(-154.64744,0.22883)
(-153.96635,0.22883)
(-153.28526,0.22883)
(-152.60417,0.22883)
(-151.92308,0.34325)
(-151.24199,0.34325)
(-150.56090,0.34325)
(-149.87981,0.34325)
(-149.19872,0.34325)
(-148.51763,0.34325)
(-147.83654,0.34325)
(-147.15545,0.34325)
(-146.47436,0.34325)
(-145.79327,0.34325)
(-145.11218,0.45767)
(-144.43109,0.45767)
(-143.75000,0.45767)
(-143.06891,0.45767)
(-142.38782,0.45767)
(-141.70673,0.45767)
(-141.02564,0.57208)
(-140.34455,0.57208)
(-139.66346,0.57208)
(-138.98237,0.57208)
(-138.30128,0.57208)
(-137.62019,0.57208)
(-136.93910,0.57208)
(-136.25801,0.57208)
(-135.57692,0.57208)
(-134.89583,0.68650)
(-134.21474,0.68650)
(-133.53365,0.68650)
(-132.85256,0.68650)
(-132.17147,0.68650)
(-131.49038,0.68650)
(-130.80929,0.68650)
(-130.12821,0.68650)
(-129.44712,0.80092)
(-128.76603,0.80092)
(-128.08494,0.80092)
(-127.40385,0.80092)
(-126.72276,0.80092)
(-126.04167,0.80092)
(-125.36058,0.80092)
(-124.67949,0.80092)
(-123.99840,0.80092)
(-123.31731,0.91533)
(-122.63622,0.91533)
(-121.95513,0.91533)
(-121.27404,0.91533)
(-120.59295,1.02975)
(-119.91186,1.02975)
(-119.23077,1.02975)
(-118.54968,1.14416)
(-117.86859,1.14416)
(-117.18750,1.14416)
(-116.50641,1.14416)
(-115.82532,1.14416)
(-115.14423,1.25858)
(-114.46314,1.25858)
(-113.78205,1.24905)
(-113.10096,1.23951)
(-112.41987,1.22998)
(-111.73878,1.22044)
(-111.05769,1.21091)
(-110.37660,1.20137)
(-109.69551,1.19184)
(-109.01442,1.18230)
(-108.33333,1.17277)
(-107.65224,1.16323)
(-106.97115,1.15370)
(-106.29006,1.14416)
(-105.60897,1.14416)
(-104.92788,1.14416)
(-104.24679,1.02975)
(-103.56571,0.91533)
(-102.88462,0.91533)
(-102.20353,0.91533)
(-101.52244,0.80092)
(-100.84135,0.68650)
(-100.16026,0.57208)
(-99.47917,0.57208)
(-98.79808,0.45767)
(-98.11699,0.34325)
(-97.43590,0.22883)
(-96.75481,0.11442)
(-96.07372,0.00000)
(-95.39263,0.00000)
(-94.71154,-0.11442)
(-94.03045,-0.22883)
(-93.34936,-0.34325)
(-92.66827,-0.45767)
(-91.98718,-0.57208)
(-91.30609,-0.57208)
(-90.62500,-0.80092)
(-89.94391,-0.91533)
(-89.26282,-1.02975)
(-88.58173,-1.14416)
(-87.90064,-1.25858)
(-87.21955,-1.37300)
(-86.53846,-1.48741)
(-85.85737,-1.71625)
(-85.17628,-1.83066)
(-84.49519,-1.94508)
(-83.81410,-2.05950)
(-83.13301,-2.17391)
(-82.45192,-2.28833)
(-81.77083,-2.40275)
(-81.08974,-2.51716)
(-80.40865,-2.63158)
(-79.72756,-2.74600)
(-79.04647,-2.86041)
(-78.36538,-2.97483)
(-77.68429,-3.08924)
(-77.00321,-3.20366)
(-76.32212,-3.20366)
(-75.64103,-3.21246)
(-74.95994,-3.22126)
(-74.27885,-3.23007)
(-73.59776,-3.23887)
(-72.91667,-3.24767)
(-72.23558,-3.25647)
(-71.55449,-3.26527)
(-70.87340,-3.27407)
(-70.19231,-3.28287)
(-69.51122,-3.29167)
(-68.83013,-3.30048)
(-68.14904,-3.30928)
(-67.46795,-3.31808)
(-66.78686,-3.20366)
(-66.10577,-3.08924)
(-65.42468,-2.97483)
(-64.74359,-2.86041)
(-64.06250,-2.74600)
(-63.38141,-2.63158)
(-62.70032,-2.51716)
(-62.01923,-2.40275)
(-61.33814,-2.28833)
(-60.65705,-2.17391)
(-59.97596,-2.05950)
(-59.29487,-1.83066)
(-58.61378,-1.71625)
(-57.93269,-1.60183)
(-57.25160,-1.48741)
(-56.57051,-1.37300)
(-55.88942,-1.14416)
(-55.20833,-0.91533)
(-54.52724,-0.68650)
(-53.84615,-0.45767)
(-53.16506,-0.34325)
(-52.48397,-0.11442)
(-51.80288,0.11442)
(-51.12179,0.22883)
(-50.44071,0.45767)
(-49.75962,0.68650)
(-49.07853,0.91533)
(-48.39744,1.14416)
(-47.71635,1.37300)
(-47.03526,1.60183)
(-46.35417,1.83066)
(-45.67308,2.05950)
(-44.99199,2.28833)
(-44.31090,2.51716)
(-43.62981,2.74600)
(-42.94872,2.86041)
(-42.26763,3.08924)
(-41.58654,3.31808)
(-40.90545,3.43249)
(-40.22436,3.66133)
(-39.54327,3.89016)
(-38.86218,4.00458)
(-38.18109,4.23341)
(-37.50000,4.34783)
(-36.81891,4.46224)
(-36.13782,4.69108)
(-35.45673,4.80549)
(-34.77564,4.91991)
(-34.09455,5.03432)
(-33.41346,5.14874)
(-32.73237,5.26316)
(-32.05128,5.26316)
(-31.37019,5.37757)
(-30.68910,5.37757)
(-30.00801,5.37757)
(-29.32692,5.37757)
(-28.64583,5.26316)
(-27.96474,5.26316)
(-27.28365,5.14874)
(-26.60256,5.03432)
(-25.92147,4.91991)
(-25.24038,4.80549)
(-24.55929,4.69108)
(-23.87821,4.46224)
(-23.19712,4.34783)
(-22.51603,4.23341)
(-21.83494,4.00458)
(-21.15385,3.89016)
(-20.47276,3.66133)
(-19.79167,3.43249)
(-19.11058,3.31808)
(-18.42949,3.20366)
(-17.74840,3.08924)
(-17.06731,2.86041)
(-16.38622,2.63158)
(-15.70513,2.51716)
(-15.02404,2.28833)
(-14.34295,2.17391)
(-13.66186,2.05950)
(-12.98077,1.83066)
(-12.29968,1.71625)
(-11.61859,1.60183)
(-10.93750,1.37300)
(-10.25641,1.25858)
(-9.57532,1.14416)
(-8.89423,1.02975)
(-8.21314,1.02975)
(-7.53205,0.91533)
(-6.85096,0.80092)
(-6.16987,0.80092)
(-5.48878,0.68650)
(-4.80769,0.68650)
(-4.12660,0.57208)
(-3.44551,0.57208)
(-2.76442,0.57208)
(-2.08333,0.57208)
(-1.40224,0.57208)
(-0.72115,0.57208)
(-0.04006,0.57208)
(0.64103,0.57208)
(1.32212,0.57208)
(2.00321,0.68650)
(2.68429,0.80092)
(3.36538,0.80092)
(4.04647,0.91533)
(4.72756,0.91533)
(5.40865,0.91533)
(6.08974,1.02975)
(6.77083,1.14416)
(7.45192,1.25858)
(8.13301,1.25858)
(8.81410,1.37300)
(9.49519,1.48741)
(10.17628,1.60183)
(10.85737,1.71625)
(11.53846,1.83066)
(12.21955,1.63759)
(12.90064,1.44451)
(13.58173,1.25143)
(14.26282,1.05835)
(14.94391,0.86527)
(15.62500,0.67220)
(16.30609,0.47912)
(16.98718,0.28604)
(17.66827,0.09296)
(18.34936,-0.10011)
(19.03045,-0.29319)
(19.71154,-0.48627)
(20.39263,-0.67935)
(21.07372,-0.87243)
(21.75481,-1.06550)
(22.43590,-1.25858)
(23.11699,-2.05950)
(23.79808,-2.86041)
(24.47917,-3.89016)
(25.16026,-4.80549)
(25.84135,-5.72082)
(26.52244,-6.63616)
(27.20353,-7.55149)
(27.88462,-8.46682)
(28.56571,-9.49657)
(29.24679,-10.52632)
(29.92788,-11.67048)
(30.60897,-12.81465)
(31.29006,-14.07323)
(31.97115,-15.33181)
(32.65224,-16.59039)
(33.33333,-17.84897)
(34.01442,-18.87872)
(34.69551,-19.79405)
(35.37660,-20.70938)
(36.05769,-21.16705)
(36.73878,-21.28146)
(37.41987,-21.16705)
(38.10096,-20.70938)
(38.78205,-19.90847)
(39.46314,-19.10755)
(40.14423,-17.96339)
(40.82532,-16.81922)
(41.50641,-15.67506)
(42.18750,-14.41648)
(42.86859,-13.27231)
(43.54968,-12.12815)
(44.23077,-10.98398)
(44.91186,-9.83982)
(45.59295,-8.58124)
(46.27404,-7.32265)
(46.95513,-6.06407)
(47.63622,-4.69108)
(48.31731,-3.31808)
(48.99840,-1.83066)
(49.67949,-0.34325)
(50.36058,0.36734)
(51.04167,1.07792)
(51.72276,1.78851)
(52.40385,2.49910)
(53.08494,14.53089)
(53.76603,12.62395)
(54.44712,13.04348)
(55.12821,13.95881)
(55.80929,14.75973)
(56.49038,15.44622)
(57.17147,15.78947)
(57.85256,16.01831)
(58.53365,16.01831)
(59.21474,16.01831)
(59.89583,16.01831)
(60.57692,15.78947)
(61.25801,15.56064)
(61.93910,14.98856)
(62.62019,14.30206)
(63.30128,12.47140)
(63.98237,11.78490)
(64.66346,11.09840)
(65.34455,10.29748)
(66.02564,9.49657)
(66.70673,8.58124)
(67.38782,7.89474)
(68.06891,7.20824)
(68.75000,6.40732)
(69.43109,5.94966)
(70.11218,5.26316)
(70.79327,4.69108)
(71.47436,4.34783)
(72.15545,3.89016)
(72.83654,3.43249)
(73.51763,2.97483)
(74.19872,2.51716)
(74.87981,2.05950)
(75.56090,1.71625)
(76.24199,1.25858)
(76.92308,0.80092)
(77.60417,0.34325)
(78.28526,-0.11442)
(78.96635,-0.57208)
(79.64744,-0.91533)
(80.32853,-1.25858)
(81.00962,-1.60183)
(81.69071,-1.83066)
(82.37179,-2.05950)
(83.05288,-2.28833)
(83.73397,-2.40275)
(84.41506,-2.51716)
(85.09615,-2.51716)
(85.77724,-2.51716)
(86.45833,-2.51716)
(87.13942,-2.51716)
(87.82051,-2.51716)
(88.50160,-2.40275)
(89.18269,-2.40275)
(89.86378,-2.28833)
(90.54487,-2.28833)
(91.22596,-2.17391)
(91.90705,-2.17391)
(92.58814,-2.05950)
(93.26923,-2.05950)
(93.95032,-1.94508)
(94.63141,-1.94508)
(95.31250,-1.94508)
(95.99359,-1.94508)
(96.67468,-1.94508)
(97.35577,-1.94508)
(98.03686,-2.05950)
(98.71795,-2.17391)
(99.39904,-2.40275)
(100.08013,-2.51716)
(100.76122,-2.74600)
(101.44231,-2.97483)
(102.12340,-3.20366)
(102.80449,-3.43249)
(103.48558,-3.66133)
(104.16667,-3.89016)
(104.84776,-4.23341)
(105.52885,-4.46224)
(106.20994,-4.80549)
(106.89103,-5.14874)
(107.57212,-5.49199)
(108.25321,-5.83524)
(108.93429,-6.17849)
(109.61538,-6.52174)
(110.29647,-6.86499)
(110.97756,-7.09382)
(111.65865,-7.43707)
(112.33974,-7.66590)
(113.02083,-7.78032)
(113.70192,-7.70751)
(114.38301,-7.63470)
(115.06410,-7.56189)
(115.74519,-7.48908)
(116.42628,-7.41627)
(117.10737,-7.34346)
(117.78846,-7.27065)
(118.46955,-7.19784)
(119.15064,-7.12503)
(119.83173,-7.05222)
(120.51282,-6.97941)
(121.19391,-6.75057)
(121.87500,-6.40732)
(122.55609,-6.06407)
(123.23718,-5.72082)
(123.91827,-5.37757)
(124.59936,-5.03432)
(125.28045,-4.69108)
(125.96154,-4.32876)
(126.64263,-3.96644)
(127.32372,-3.60412)
(128.00481,-3.24180)
(128.68590,-2.87948)
(129.36699,-2.51716)
(130.04808,-2.15484)
(130.72917,-1.79252)
(131.41026,-1.43021)
(132.09135,-1.06789)
(132.77244,-0.70557)
(133.45353,-0.34325)
(134.13462,0.00000)
(134.81571,0.34325)
(135.49679,0.68650)
(136.17788,1.02975)
(136.85897,1.37300)
(137.54006,1.71625)
(138.22115,1.94508)
(138.90224,2.28833)
(139.58333,2.63158)
(140.26442,2.86041)
(140.94551,3.08924)
(141.62660,3.43249)
(142.30769,3.66133)
(142.98878,3.89016)
(143.66987,4.11899)
(144.35096,4.34783)
(145.03205,4.57666)
(145.71314,4.80549)
(146.39423,4.91991)
(147.07532,5.14874)
(147.75641,5.26316)
(148.43750,5.37757)
(149.11859,5.49199)
(149.79968,5.60641)
(150.48077,5.72082)
(151.16186,5.83524)
(151.84295,5.94966)
(152.52404,5.94966)
(153.20513,6.06407)
(153.88622,6.06407)
(154.56731,6.06407)
(155.24840,5.94966)
(155.92949,5.94966)
(156.61058,5.94966)
(157.29167,5.83524)
(157.97276,5.83524)
(158.65385,5.72082)
(159.33494,5.72082)
(160.01603,5.60641)
(160.69712,5.49199)
(161.37821,5.49199)
(162.05929,5.37757)
(162.74038,5.26316)
(163.42147,5.14874)
(164.10256,5.03432)
(164.78365,4.91991)
(165.46474,4.80549)
(166.14583,4.69108)
(166.82692,4.57666)
(167.50801,4.46224)
(168.18910,4.34783)
(168.87019,4.23341)
(169.55128,4.11899)
(170.23237,4.00458)
(170.91346,3.89016)
(171.59455,3.77574)
(172.27564,3.54691)
(172.95673,3.43249)
(173.63782,3.31808)
(174.31891,3.20366)
(175.00000,3.08924)
(175.68109,2.97483)
(176.36218,2.74600)
(177.04327,2.63158)
(177.72436,2.51716)
(178.40545,2.40275)
(179.08654,2.17391)
(179.76763,2.17391)
(180.44872,2.05950)
(181.12981,1.94508)
(181.81090,1.83066)
(182.49199,1.71625)
(183.17308,1.60183)
(183.85417,1.48741)
(184.53526,1.37300)
(185.21635,1.37300)
(185.89744,1.25858)
(186.57853,1.14416)
(187.25962,1.02975)
(187.94071,0.91533)
(188.62179,0.80092)
(189.30288,0.80092)
(189.98397,0.68650)
(190.66506,0.57208)
(191.34615,0.57208)
(192.02724,0.45767)
(192.70833,0.45767)
(193.38942,0.34325)
(194.07051,0.34325)
(194.75160,0.22883)
(195.43269,0.22883)
(196.11378,0.11442)
(196.79487,0.11442)
(197.47596,0.11442)
(198.15705,0.00000)
(198.83814,-0.11442)
(199.51923,-0.11442)
(200.20032,-0.11442)
(200.88141,-0.11442)
(201.56250,-0.11442)
(202.24359,-0.22883)
(202.92468,-0.22883)
(203.60577,-0.22883)
(204.28686,-0.22883)
(204.96795,-0.22883)
(205.64904,-0.34325)
(206.33013,-0.34325)
(207.01122,-0.34325)
(207.69231,-0.34325)
(208.37340,-0.34325)
(209.05449,-0.34325)
(209.73558,-0.45767)
(210.41667,-0.45767)
(211.09776,-0.45767)
(211.77885,-0.45767)
(212.45994,-0.45767)
(213.14103,-0.45767)
(213.82212,-0.45767)
(214.50321,-0.45767)
(215.18429,-0.45767)
(215.86538,-0.45767)
(216.54647,-0.45767)
(217.22756,-0.45767)
(217.90865,-0.45767)
(218.58974,-0.45767)
(219.27083,-0.45767)
(219.95192,-0.45767)
(220.63301,-0.45767)
(221.31410,-0.45767)
(221.99519,-0.45767)
(222.67628,-0.45767)
(223.35737,-0.45767)
(224.03846,-0.45767)
(224.71955,-0.45767)
(225.40064,-0.34325)
(226.08173,-0.34325)
(226.76282,-0.34325)
(227.44391,-0.34325)
(228.12500,-0.34325)
(228.80609,-0.34325)
(229.48718,-0.22883)
(230.16827,-0.22883)
(230.84936,-0.22883)
(231.53045,-0.22883)
(232.21154,-0.22883)
(232.89263,-0.22883)
(233.57372,-0.22883)
(234.25481,-0.22883)
(234.93590,-0.22883)
(235.61699,-0.11442)
(236.29808,-0.11442)
(236.97917,-0.11442)
(237.66026,-0.11442)
(238.34135,-0.11442)
(239.02244,-0.11442)
(239.70353,-0.11442)
(240.38462,0.00000)
(241.06571,0.00000)
(241.74679,0.00000)
(242.42788,0.00000)
(243.10897,0.00000)
(243.79006,0.11442)
(244.47115,0.11442)
(245.15224,0.11442)
(245.83333,0.11442)
(246.51442,0.22883)
(247.19551,0.22883)
(247.87660,0.22883)
(248.55769,0.22883)
(249.23878,0.22883)
(249.91987,0.22883)
(250.60096,0.22883)
(251.28205,0.34325)
(251.96314,0.34325)
(252.64423,0.34325)
(253.32532,0.34325)
(254.00641,0.34325)
(254.68750,0.34325)
(255.36859,0.34325)
(256.04968,0.45767)
(256.73077,0.45767)
(257.41186,0.45767)
(258.09295,0.45767)
(258.77404,0.45767)
(259.45513,0.57208)
(260.13622,0.57208)
(260.81731,0.57208)
(261.49840,0.57208)
(262.17949,0.57208)
(262.86058,0.57208)
(263.54167,0.57208)
(264.22276,0.57208)
(264.90385,0.68650)
(265.58494,0.68650)
(266.26603,0.68650)
(266.94712,0.68650)
(267.62821,0.80092)
(268.30929,0.80092)
(268.99038,0.80092)
(269.67147,0.80092)
(270.35256,0.80092)
(271.03365,0.91533)
(271.71474,0.91533)
(272.39583,0.91533)
(273.07692,0.91533)
(273.75801,0.91533)
(274.43910,0.91533)
(275.12019,0.91533)
(275.80128,1.02975)
(276.48237,1.02975)
(277.16346,1.02975)
(277.84455,1.02975)
(278.52564,1.02975)
(279.20673,1.02975)
(279.88782,1.14416)
(280.56891,1.14416)
(281.25000,1.14416)
(281.93109,1.14416)
(282.61218,1.14416)
(283.29327,1.14416)
(283.97436,1.14416)
(284.65545,1.25858)
(285.33654,1.25858)
(286.01763,1.25858)
(286.69872,1.25858)
(287.37981,1.25858)
(288.06090,1.25858)
(288.74199,1.25858)
(289.42308,1.25858)
(290.10417,1.25858)
(290.78526,1.25858)
(291.46635,1.25858)
(292.14744,1.25858)
(292.82853,1.25858)
(293.50962,1.25858)
(294.19071,1.25858)
(294.87179,1.25858)
(295.55288,1.25858)
(296.23397,1.25858)
(296.91506,1.25858)
(297.59615,1.37300)
(298.27724,1.37300)
(298.95833,1.37300)
(299.63942,1.37300)
(300.32051,1.37300)
(301.00160,1.37300)
(301.68269,1.37300)
(302.36378,1.37300)
(303.04487,1.37300)
(303.72596,1.37300)
(304.40705,1.37300)
(305.08814,1.37300)
(305.76923,1.37300)
(306.45032,1.48741)
(307.13141,1.48741)
(307.81250,1.48741)
(308.49359,1.48741)
(309.17468,1.48741)
(309.85577,1.48741)
(310.53686,1.48741)
(311.21795,1.48741)
(311.89904,1.48741)
(312.58013,1.48741)
(313.26122,1.48741)
(313.94231,1.48741)
(314.62340,1.48741)
(315.30449,1.48741)
(315.98558,1.48741)
(316.66667,1.60183)
(317.34776,1.60183)
(318.02885,1.60183)
(318.70994,1.60183)
(319.39103,1.71625)
(320.07212,1.71625)
(320.75321,1.71625)
(321.43429,1.71625)
(322.11538,1.71625)
(322.79647,1.83066)
(323.47756,1.83066)
(324.15865,1.83066)
(324.83974,1.83066)
(325.52083,1.94508)
(326.20192,2.05950)
(326.88301,2.05950)
(327.56410,2.05950)
(328.24519,2.17391)
(328.92628,2.17391)
(329.60737,2.17391)
(330.28846,2.28833)
(330.96955,2.40275)
(331.65064,2.40275)
(332.33173,2.51716)
(333.01282,2.51716)
(333.69391,2.63158)
(334.37500,2.63158)
(335.05609,2.74600)
(335.73718,2.74600)
(336.41827,2.74600)
(337.09936,2.86041)
(337.78045,2.86041)
(338.46154,2.84481)
(339.14263,2.82921)
(339.82372,2.81361)
(340.50481,2.79800)
(341.18590,2.78240)
(341.86699,2.76680)
(342.54808,2.75120)
(343.22917,2.73559)
(343.91026,2.71999)
(344.59135,2.70439)
(345.27244,2.68879)
(345.95353,2.67318)
(346.63462,2.65758)
(347.31571,2.64198)
(347.99679,2.62638)
(348.67788,2.61078)
(349.35897,2.59517)
(350.04006,2.57957)
(350.72115,2.56397)
(351.40224,2.54837)
(352.08333,2.53276)
(352.76442,2.51716)
(353.44551,2.40275)
(354.12660,2.17391)
(354.80769,2.05950)
(355.48878,1.83066)
(356.16987,1.60183)
(356.85096,1.48741)
(357.53205,1.25858)
(358.21314,1.02975)
(358.89423,0.80092)
(359.57532,0.68650)
(360.25641,0.45767)
(360.93750,0.34325)
(361.61859,0.22883)
(362.29968,0.11442)
(362.98077,0.00000)
(363.66186,-0.11442)
(364.34295,-0.11442)
(365.02404,-0.11442)
(365.70513,0.00000)
(366.38622,0.11442)
(367.06731,0.22883)
(367.74840,0.34325)
(368.42949,0.57208)
(369.11058,0.80092)
(369.79167,1.02975)
(370.47276,1.25858)
(371.15385,1.48741)
(371.83494,1.71625)
(372.51603,1.94508)
(373.19712,2.17391)
(373.87821,2.40275)
(374.55929,2.63158)
(375.24038,2.86041)
(375.92147,2.97483)
(376.60256,3.20366)
(377.28365,3.31808)
(377.96474,3.43249)
(378.64583,3.54691)
(379.32692,3.54691)
(380.00801,3.54691)
(380.68910,3.54691)
(381.37019,3.54691)
(382.05128,3.43249)
(382.73237,3.31808)
(383.41346,3.08924)
(384.09455,2.97483)
(384.77564,2.74600)
(385.45673,2.40275)
(386.13782,2.17391)
(386.81891,1.83066)
(387.50000,1.60183)
(388.18109,1.25858)
(388.86218,1.02975)
(389.54327,0.68650)
(390.22436,0.34325)
(390.90545,0.00000)
(391.58654,-0.22883)
(392.26763,-0.57208)
(392.94872,-0.91533)
(393.62981,-1.14416)
(394.31090,-1.48741)
(394.99199,-1.83066)
(395.67308,-2.05950)
(396.35417,-2.40275)
(397.03526,-2.74600)
(397.71635,-2.97483)
(398.39744,-3.20366)
(399.07853,-3.43249)
(399.75962,-3.66133)
(400.44071,-3.89016)
(401.12179,-4.11899)
(401.80288,-4.34783)
(402.48397,-4.57666)
(403.16506,-4.80549)
(403.84615,-5.03432)
(404.52724,-5.14874)
(405.20833,-5.26316)
(405.88942,-5.37757)
(406.57051,-5.49199)
(407.25160,-5.49199)
(407.93269,-5.60641)
(408.61378,-5.60641)
(409.29487,-5.60641)
(409.97596,-5.60641)
(410.65705,-5.49199)
(411.33814,-5.49199)
(412.01923,-5.37757)
(412.70032,-5.26316)
(413.38141,-5.14874)
(414.06250,-5.03432)
(414.74359,-4.91991)
(415.42468,-4.80549)
(416.10577,-4.69108)
(416.78686,-4.57666)
(417.46795,-4.46224)
(418.14904,-4.34783)
(418.83013,-4.23341)
(419.51122,-4.00458)
(420.19231,-3.77574)
(420.87340,-3.54691)
(421.55449,-3.43249)
(422.23558,-3.20366)
(422.91667,-3.08924)
(423.59776,-3.00343)
(424.27885,-2.91762)
(424.95994,-2.83181)
(425.64103,-2.74600)
(426.32212,-2.66018)
(427.00321,-2.57437)
(427.68429,-2.48856)
(428.36538,-2.40275)
(429.04647,-2.31693)
(429.72756,-2.23112)
(430.40865,-2.14531)
(431.08974,-2.05950)
(431.77083,-1.97368)
(432.45192,-1.88787)
(433.13301,-1.80206)
(433.81410,-1.71625)
(434.49519,-1.63043)
(435.17628,-1.54462)
(435.85737,-1.45881)
(436.53846,-1.37300)
(437.21955,-1.28719)
(437.90064,-1.20137)
(438.58173,-1.11556)
(439.26282,-1.02975)
(439.94391,-0.94394)
(440.62500,-0.85812)
(441.30609,-0.77231)
(441.98718,-0.68650)
(442.66827,-0.68650)
(443.34936,-0.80092)
(444.03045,-0.80092)
(444.71154,-0.80092)
(445.39263,-0.91533)
(446.07372,-1.02975)
(446.75481,-1.02975)
(447.43590,-1.02975)
(448.11699,-1.02975)
(448.79808,-1.14416)
(449.47917,-1.14416)
(450.16026,-1.14416)
(450.84135,-1.25858)
(451.52244,-1.25858)
(452.20353,-1.25858)
(452.88462,-1.25858)
(453.56571,-1.25858)
(454.24679,-1.25858)
(454.92788,-1.25858)
(455.60897,-1.25858)
(456.29006,-1.25858)
(456.97115,-1.25858)
(457.65224,-1.25858)
(458.33333,-1.25858)
(459.01442,-1.25858)
(459.69551,-1.14416)
(460.37660,-1.14416)
(461.05769,-1.14416)
(461.73878,-1.02975)
(462.41987,-1.02975)
(463.10096,-0.91533)
(463.78205,-0.91533)
(464.46314,-0.80092)
(465.14423,-0.80092)
(465.82532,-0.68650)
(466.50641,-0.68650)
(467.18750,-0.57208)
(467.86859,-0.45767)
(468.54968,-0.45767)
(469.23077,-0.22883)
(469.91186,-0.22883)
(470.59295,-0.22883)
(471.27404,-0.11442)
(471.95513,0.00000)
(472.63622,0.00000)
(473.31731,0.11442)
(473.99840,0.22883)
(474.67949,0.22883)
(475.36058,0.34325)
(476.04167,0.45767)
(476.72276,0.45767)
(477.40385,0.57208)
(478.08494,0.68650)
(478.76603,0.80092)
(479.44712,0.91533)
(480.12821,1.02975)
(480.80929,1.14416)
(481.49038,1.14416)
(482.17147,1.25858)
(482.85256,1.37300)
(483.53365,1.48741)
(484.21474,1.60183)
(484.89583,1.71625)
(485.57692,1.83066)
(486.25801,1.93237)
(486.93910,2.03407)
(487.62019,2.13577)
(488.30128,2.23748)
(488.98237,2.33918)
(489.66346,2.44088)
(490.34455,2.54259)
(491.02564,2.64429)
(491.70673,2.74600)
(492.38782,2.84770)
(493.06891,2.94940)
(493.75000,3.05111)
(494.43109,3.15281)
(495.11218,3.25451)
(495.79327,3.35622)
(496.47436,3.45792)
(497.15545,3.55962)
(497.83654,3.66133)
(498.51763,3.77574)
(499.19872,3.89016)
(499.87981,4.00458)
(500.56090,4.00458)
(501.24199,4.11899)
(501.92308,4.11899)
(502.60417,4.23341)
(503.28526,4.23341)
(503.96635,4.23341)
(504.64744,4.23341)
(505.32853,4.23341)
(506.00962,4.23341)
(506.69071,4.23341)
(507.37179,4.23341)
(508.05288,4.23341)
(508.73397,4.23341)
(509.41506,4.23341)
(510.09615,4.23341)
(510.77724,4.23341)
(511.45833,4.23341)
(512.13942,4.11899)
(512.82051,4.11899)
(513.50160,4.00458)
(514.18269,4.00458)
(514.86378,3.89016)
(515.54487,3.77574)
(516.22596,3.77574)
(516.90705,3.66133)
(517.58814,3.54691)
(518.26923,3.54691)
(518.95032,3.43249)
(519.63141,3.31808)
(520.31250,3.20366)
(520.99359,3.20366)
(521.67468,3.08924)
(522.35577,2.97483)
(523.03686,2.97483)
(523.71795,2.86041)
(524.39904,2.74600)
(525.08013,2.63158)
(525.76122,2.63158)
(526.44231,2.51716)
(527.12340,2.40275)
(527.80449,2.40275)
(528.48558,2.28833)
(529.16667,2.17391)
(529.84776,2.05950)
(530.52885,2.05950)
(531.20994,1.94508)
(531.89103,1.83066)
(532.57212,1.83066)
(533.25321,1.71625)
(533.93429,1.71625)
(534.61538,1.60183)
(535.29647,1.48741)
(535.97756,1.48741)
(536.65865,1.37300)
(537.33974,1.37300)
(538.02083,1.25858)
(538.70192,1.25858)
(539.38301,1.14416)
(540.06410,1.14416)
(540.74519,1.14416)
(541.42628,1.02975)
(542.10737,1.02975)
(542.78846,1.02975)
(543.46955,0.91533)
(544.15064,0.91533)
(544.83173,0.91533)
(545.51282,0.80092)
(546.19391,0.80092)
(546.87500,0.80092)
(547.55609,0.68650)
(548.23718,0.68650)
(548.91827,0.68650)
(549.59936,0.57208)
(550.28045,0.57208)
(550.96154,0.57208)
(551.64263,0.45767)
(552.32372,0.45767)
(553.00481,0.45767)
(553.68590,0.34325)
(554.36699,0.34325)
(555.04808,0.34325)
(555.72917,0.22883)
(556.41026,0.22883)
(557.09135,0.22883)
(557.77244,0.11442)
(558.45353,0.11442)
(559.13462,0.11442)
(559.81571,0.11442)
(560.49679,0.11442)
(561.17788,0.00000)
(561.85897,0.00000)
(562.54006,0.00000)
(563.22115,0.00000)
(563.90224,0.00000)
(564.58333,-0.11442)
(565.26442,-0.11442)
(565.94551,-0.11442)
(566.62660,-0.11442)
(567.30769,-0.11442)
(567.98878,-0.11442)
(568.66987,-0.22883)
(569.35096,-0.22883)
(570.03205,-0.22883)
(570.71314,-0.22883)
(571.39423,-0.22883)
(572.07532,-0.22883)
(572.75641,-0.22883)
(573.43750,-0.22883)
(574.11859,-0.22883)
(574.79968,-0.22883)
(575.48077,-0.22883)
(576.16186,-0.22883)
(576.84295,-0.22883)
(577.52404,-0.22883)
(578.20513,-0.22883)
(578.88622,-0.22883)
(579.56731,-0.22883)
(580.24840,-0.22883)
(580.92949,-0.22883)
(581.61058,-0.22883)
(582.29167,-0.22883)
(582.97276,-0.22883)
(583.65385,-0.22883)
(584.33494,-0.22883)
(585.01603,-0.22883)
(585.69712,-0.22883)
(586.37821,-0.22883)
(587.05929,-0.22883)
(587.74038,-0.22883)
(588.42147,-0.11442)
(589.10256,-0.11442)
(589.78365,-0.11442)
(590.46474,-0.11442)
(591.14583,-0.22883)
(591.82692,-0.22883)
(592.50801,-0.22883)
(593.18910,-0.22883)
(593.87019,-0.22883)
(594.55128,-0.11442)
(595.23237,-0.11442)
(595.91346,-0.11442)
(596.59455,-0.22883)
(597.27564,-0.22883)
(597.95673,-0.22883)
(598.63782,-0.22883)
(599.31891,-0.22883)
};


==> figures/signals/scg_waveform_events.tex <==
\coordinate (MC) at (16.00000,0.56589);
\coordinate (AO) at (59.00000,16.01831);
\coordinate (AC) at (348.00000,2.62630);
\coordinate (MO) at (437.00000,-1.31485);


==> figures/signals/scg_waveform_simple.tex <==
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[x=0.31pt,y=2.4pt,font=\scriptsize]
\draw[black!65,line width=0.45pt] (-250,20)--(-250,-30)--(600,-30);
\foreach \y in {-30,-20,-10,0,10,20}{%
  \draw[black!65,line width=0.4pt] (-250,\y)--(-260,\y);
  \node[anchor=east,inner sep=2pt] at (-260,\y) {\y};
}
\foreach \x in {-200,-100,0,100,200,300,400,500,600}{%
  \draw[black!65,line width=0.4pt] (\x,-30)--(\x,-31.3);
  \node[anchor=north,inner sep=3pt] at (\x,-31.3) {\x};
}
\node[rotate=90,anchor=south] at (-352,-5) {Acceleration (mg)};
\node[anchor=north] at (175,-39) {Time relative to ECG R-peak (ms)};
\begin{scope}
\clip (-250,-30) rectangle (600,20);
\input{figures/signals/scg_waveform_coordinates}
\end{scope}
\input{figures/signals/scg_waveform_events}
\foreach \event in {MC,AO,AC,MO}{%
  \filldraw[fill=white,draw=navy,line width=0.7pt] (\event) circle[radius=1.5pt];
}
\draw[navy,line width=0.5pt] (MC)--++(-12pt,14pt) node[above,font=\small\bfseries] {MC};
\draw[navy,line width=0.5pt] (AO)--++(5pt,15pt) node[above,font=\small\bfseries] {AO};
\draw[navy,line width=0.5pt] (AC)--++(-3pt,15pt) node[above,font=\small\bfseries] {AC};
\draw[navy,line width=0.5pt] (MO)--++(10pt,13pt) node[above,font=\small\bfseries] {MO};
\end{tikzpicture}}

